Challenging Language-Dependent Segmentation for Arabic: An Application to Machine Translation and Part-of-Speech Tagging

Word segmentation plays a pivotal role in improving any Arabic NLP application. Therefore, a lot of research has been spent in improving its accuracy. Off-the-shelf tools, however, are: i) complicated to use and ii) domain/dialect dependent. We explore three language-independent alternatives to morphological segmentation using: i) data-driven sub-word units, ii) characters as a unit of learning, and iii) word embeddings learned using a character CNN (Convolution Neural Network). On the tasks of Machine Translation and POS tagging, we found these methods to achieve close to, and occasionally surpass state-of-the-art performance. In our analysis, we show that a neural machine translation system is sensitive to the ratio of source and target tokens, and a ratio close to 1 or greater, gives optimal performance.

==> defs.tex <==
% DEFINITIONS of the paper (use \newcommand instead of \def)

%%math

\DeclareMathOperator \real{\mathbb{R}}
\DeclareMathOperator \softmax{softmax}

\DeclareMathOperator*{\argmax}{\arg\!\max}
\def\layersep{2.5cm}
%%%hyphenations

%%% colors
\newcommand{\comm}[1]{\textcolor{purple}{\noindent #1}}
\newcommand{\alert}[1]{\textcolor{red}{\noindent$\Rightarrow$ #1}}


\newcommand{\nadir}[1]{\textcolor{red}{#1}}
\newcommand{\shafiq}[1]{\textcolor{blue}{#1}}
\newcommand{\kamla}[1]{\textcolor{magenta}{#1}}
\newcommand{\hassan}[1]{\textcolor{green}{#1}}
\newcommand{\ahmed}[1]{\textcolor{yellow}{#1}}


%%% MT metrics and variants
\newcommand{\bleu}{\nobreak{BLEU}}
\newcommand{\nist}{\nobreak{NIST}}

%%% MT components

\newcommand{\ind}{\nobreak{-{\sc in}}}
\newcommand{\outd}{\nobreak{-{\sc out}}}
\newcommand{\catd}{\nobreak{-{\sc cat}}}
\newcommand{\muld}{\nobreak{-{\sc mul}}}
\newcommand{\intd}{\nobreak{-{\sc int}}}
\newcommand{\adpd}{\nobreak{-{\sc adp}}}


\newcommand{\lm}{\nobreak{LM}}
\newcommand{\lmin}{\nobreak{LM-{\sc in}}}
\newcommand{\lmout}{\nobreak{LM-{\sc out}}}
\newcommand{\lmcat}{\nobreak{LM-{\sc cat}}}
\newcommand{\lmmul}{\nobreak{LM-{\sc mul}}}
\newcommand{\lmint}{\nobreak{LM-{\sc int}}}

\newcommand{\tm}{\nobreak{TM}}
\newcommand{\tmin}{\nobreak{TM-{\sc in}}}
\newcommand{\tmout}{\nobreak{TM-{\sc out}}}
\newcommand{\tmcat}{\nobreak{TM-{\sc cat}}}
\newcommand{\tmint}{\nobreak{TM-{\sc int}}}
\newcommand{\tmmul}{\nobreak{TM-{\sc mul}}}

%%% language pairs
\newcommand{\deen}{\nobreak{\sc de-en}}
\newcommand{\esen}{\nobreak{\sc es-en}}
\newcommand{\fren}{\nobreak{\sc fr-en}}
\newcommand{\aren}{\nobreak{\sc ar-en}}

%%% corpora
\newcommand{\wmte}{\nobreak{WMT11}}
\newcommand{\wmtt}{\nobreak{WMT12}}

%%% inline lists
\newcommand{\Ni}{({\em i})~}
\newcommand{\Nii}{({\em ii})~}
\newcommand{\Niii}{({\em iii})~}
\newcommand{\Niv}{({\em iv})~}
\newcommand{\Nv}{({\em v})~}
\newcommand{\Nvi}{({\em vi})~}


\newcommand{\Na}{({\em a})~}
\newcommand{\Nb}{({\em b})~}
\newcommand{\Nc}{({\em c})~}


\newcommand{\srccon}{({\em $S_i$})~}

==> discussion.tex <==
\section{Discussion}

Though BPE performed well for machine translation, there are a few reservations that we would like to discuss here. Since main goal of the algorithm is to compress data and segmentation comes as a by product, it often produces different segmentations of a root word when occurred in different morphological forms. For example, words \emph{driven} and \emph{driving} are segmented as \emph{driv en} and \emph{drivi ng} respectively. This adds ambiguity to the data and may result in unexpected translation errors. Another limitation of BPE is that at test time, it may divide the unknown words to semantically different known sub-word units which resulted in a semantically wrong translation. For example, the word ``\<قطر>'' is unknown to our vocabulary. BPE segmented it into known units which ended up translated to \emph{courage}. One solution to this problem is; at test time, we apply BPE to those words only which were known to the full vocabulary of the training corpus. In this way, the sub-word units created by BPE for the word are already seen in similar context during training and model has learned to translate them correctly. The downside of this method is that it limits BPE's power to segment unknown words to their correct sub-word units and outputs them as \emph{UNK} in translation.

==> introduction-bak.tex <==
\section{Introduction}

% Arabic language is widely used in the middle east and in Africa as one of the main languages for communication.
% \alert{ND: The above is common knowledge and the first line of paragraph should represent what the paragraph is about}
%\alert{HS: can we mention somewhere that we are not claiming to learn morphological segmentation but segmentation which is good enough for NLP applications to perform well}
%Morphological 
Arabic word segmentation has shown to improve the quality of NLP tasks such as machine translation \cite{habash:naacl06,almahairi:arxiv},
%,sajjad-etal:iwslt13}, 
POS tagging \cite{Habash:2005:ATP:1219840.1219911,Diab:2004:ATA:1613984.1614022}, and information retrieval \cite{aljlayl:2002}. 
%
%Arabic word segmentation is a %crucial
%crucial % foremost obligatory 
%step %for processing Arabic  in various 
%in many NLP tasks and has shown to improve , %ranging from
%such as % be it %
%part-of-speech (POS) tagging, %and 
%parsing, %to 
%information retrieval, %and 
%and machine translation. 
Morphological segmentation splits words into morphemes.  
For example, the Arabic word `\mbox{`\textit{wktAbnA}''}
``\<وكتابنا>'' (gloss: and our book) is composed of a prefix \mbox{``\textit{w}''} ``\<و>'' (and), a stem ``\textit{ktAb}'' ``\<كتاب>'' (book), and a possessive pronoun \mbox{``\textit{nA}''} ``\<نا>'' (our). The task of a morphological 
segmenter is to split the word into its stem and affixes, for example: \mbox{``\textit{w+ ktAb +nA}''} ``\<و+ كتاب +نا>''. 
%Segmenting words into smaller units deals with two main challenges: data sparsity and sense ambiguity. 


%
%Morphology-aware 
%Arabic morphological word segmentation has shown to %give improvements of 
%improve the quality of NLP applications such as machine translation \cite{habash:naacl06,almahairi:arxiv},
%,sajjad-etal:iwslt13}, 
%POS tagging \cite{Habash:2005:ATP:1219840.1219911,Diab:2004:ATA:1613984.1614022}, and information retrieval \cite{aljlayl:2002}. % In machine translation, it improves the quality by 2-3 BLEU points \cite{sajjad-etal:iwslt13}.
%,almahairi:arxiv},  

A considerable amount of research has 
been spent on Arabic morphological segmentation in the past two decades ranging from rule-based analyzers  \cite{beesley1989two,beesley1996arabic} %,buckwalter2002buckwalter,khoja2001apt}, 
%light stemmers \cite{aljlayl2002arabic,darwish2007adapting}, 
to statistical segmenters \cite{darwish2002building,habash2009mada+,%diab2009second,darwish2014using,
pasha2014madamira}.  
The latter class is considered to be state-of-the-art with reported segmentation accuracy of above 98\%. %The morphological segmenter splits a word into linguistically correct morphemes.
%These tools typically %i) normalize Arabic by mapping different variations of a character to one form and ii)
%segment words into constituent prefix(es), stem, and suffix(es). \alert{FD: We already mentioned in previous paragraph that the job of segmenter is to .., we can remove this line} 
%Almost all of these tools 
%them 
%rely on manually-crafted linguistic resources. \alert{FD: Do we need to mention this? This implies that there are tools which are not based on linguistic resources like bpe, and I guess a reviewer might want to atleast see the performance of such a technique since its directly comparable to bpe} 

% For example, the word ``wktAbnA''
% ``\<وكتابنا>'' (gloss: ``and our book'') is composed of the prefix ``w'' ``\<و>'' (and), stem ``ktAb'' ``\<كتاب>'' (book), and a possessive pronoun ``nA'' ``\<نا>'' (our). The task of the segmenter is to split the word into ``w+ ktAb +nA'' ``\<و+ كتاب +نا>''.

%In this work, we analyzed the usefulness of morphology-aware segmentation 

%
%Previous work on Arabic to English machine translation showed that morphology-aware segmentation of Arabic improved the system by more than 3 BLEU points **cite. These gains are consistent for both, the phrase-based system and the neural machine translation (NMT) system. 
% 
%\alert{YB: I'm not so clear about the rest of this paragraph; consider removing it \\ HS: we may remove it. I put it thinking if we have some analysis on infrequent word segmentation}
%However, it is not clear whether the improvement \sout{comes} \alert{is} due to \sout{the} linguistically correct segmentation, which improves \sout{the} word-level mapping between Arabic and other language or \sout{it is} because of the improved coverage of the system %and reduce the problem of data sparseness. 
%by virtue of addressing the problem of data sparsity.
%
%suffer the problem of data sparseness. Segmentation divides words into linguistically formed smaller units which improves the coverage of the system and helps to reduce the problem of data sparseness. 
%

%Aside from 
Despite the %benefit of using
gains obtained by %
from using 
morphological segmentation, there are several caveats to %relying on such 
using these tools. Firstly, morphological segmenters make
%the pipeline of NLP tools like machine translation 
the training pipeline %complicated and 
cumbersome, as they %introduce 
come with complicated pre-processing 
and potentially % (and 
additional post-processing (e.g. in the case of English-to-Arabic translation~\cite{Kholy:Habash:2012}). More importantly, %however, 
these tools are dialect- and domain-specific. A segmenter trained for Modern Standard Arabic performs significantly worse on dialectal Arabic \cite{Habash13morph}, or when it 
is applied %comes 
to a new domain (such as informal text, medical terms or patents).

%and their performance drops significantly when used on a new domains (such as medical %text  and educational domains). %text. 

In this work, we explore whether we can avoid the
%get rid of 
%off-the-shelf 
\emph{language-dependent} pre/post-processing components and learn segmentation directly from the training data %that is 
being used for the given task. % itself. 
We investigate data-driven alternatives to morphological 
%word 
segmentation using i) 
unsupervised sub-word units obtained using % with data driven-based method -- 
byte-pair encoding 
\cite{sennrich-haddow-birch:2016:P16-12}, 
ii) purely character-based segmentation \cite{lingTDB15}, 
%({\tt Char}), 
and iii) a convolutional neural network %({\tt cCNN})
over characters~\cite{KimAAAI1612489}. 

%In this work, we aim at achieving comparable translation quality as produced using morphology-aware segmentation, in addition bring the benefit of language independent pipeline. To achieve this,  we investigate several alternatives to morphology-aware segmentation in a neural machine translation pipeline, including unsupervised segmentation of infrequent words with byte-pair encoding ({\tt BPE}) \cite{sennrich-haddow-birch:2016:P16-12}, a convolutional neural network ({\tt cCNN}) over characters~\cite{KimAAAI1612489}, and a fully character-level encoding.  
%We compared it against a system trained on unsegmented Arabic with infrequent words handled through data driven segmentation. 
%\alert{ND: The below paragraph is good, but can say this later}
%The {\tt BPE} segmentation is particularly interesting because of the fact that it focuses on reducing out-of-vocabulary words and better modeling of infrequent words by splitting them into frequent sub-word units instead of linguistically correct units. Sub-word units have been successfully used in different NLP tasks such as POS-tagging~\cite{SantosZ14}, name-entity recognition~\cite{SantosG15}, parsing \cite{ballesteros-dyer-smith:2015:EMNLP}, word representations \cite{ChenXLSL15} and machine translation \cite{sennrich-lexi-bary:2016:ACL2016,costajussa-fonollosa:2016:P16-2} from the perspective of modeling infrequent words better. Here we explore different sub-word strategies with a goal of exploring them as an alternative to Arabic word-segmentation.
We evaluate these 
%segmentation 
techniques on the tasks of machine translation and POS tagging and compared them against state-of-the-art Arabic morphological segmenters MADAMIRA \cite{PASHA14.593} and Farasa \cite{abdelali-EtAl:2016:N16-3}. Our results show that language-independent 
%the data-driven 
%segmentation
processing
performs close to and sometimes surpasses morphology-aware segmenters. %for the tasks in hand. 
On the machine translation task, % {\tt BPE} %performs comparable to the morphology-aware segmentation
byte-pair encoding ({\tt BPE})
performs the best among the three methods, achieving very similar performance to morphology-aware segmentation in the Arabic-to-English direction. %, indicating that most of the gains come from better handling of infrequent words. Character-based methods were worse than B
Character-based methods give significant improvement compared to unsegmented data, but perform slightly worse than {\tt BPE}
on translation. 
On the contrary, character-based methods perform better on the task of POS tagging, 
reaching %giving 
an accuracy of $95.9\%$, only $1.3\%$ worse 
than %compared to the 
morphological segmentation. %In addition, 
We also analyzed the effect of segmentation granularity of Arabic on the quality of machine translation. We observed that a neural machine translation system is sensitive to source/target token ratio and performs best when this ratio is close to or greater \mbox{than 1}.
%The remainder of this paper is organized as follows: Section \ref{sec:segmentation} summarizes segmentation approaches that we explored. Section \ref{sec:experiments} presents the experiments. %We provide an analysis of the segmentations in Section \ref{sec:analysis}. Section \ref{sec:conclusion} concludes.

%\alert{YB: consider removing the last bit about how the paper is organized.}

%Our machine translation results showed that unsupervised segmentation using {\tt BPE} performs comparable to the morphology-aware segmentation in Arabic-to-English direction, indicating that most of the gains come from better handling of infrequent words. We also found that fully character-level encoding and character CNN-based method improved performance over the unsegmented system but do not guarantee a high quality translation system. In the English-to-Arabic translation direction, these methods performed poorly. The BPE-based system performed lower by 0.5 BLEU points compared to the best morphology-aware system in this direction. However, it brought the advantage of language independent pre- and post-processing.
%Our results on using sub-word units for Arabic POS tagging also showed an improvement of 4 points when compared with using unsegmented text and is lower by only 1.3 points from using morphology-aware segmentation.

%

%\alert{ND: I think below is still speculative and we don't have very conclusive empirical evidence to pitch it strongly in the intro. Also how would you optimize OP for POS tagging, IR? Commenting it}
%We analyzed the BPE-based segmentation with varying it's hyper-parameter. We showed that neural machine translation system performs better with a source to target ratio of 1 or greater provided that the boundary conditions (no segmentation, character-level segmentation) are avoided.

%Interestingly, the contributions from the two segmentation approaches are complimentary to some extent.  We also find that fully character-level encoding performs the best, but \sout{observe high computational costs in training it} \alert{it is computationally expensive to train these models}. 

% We also perform experiments translating into Arabic and got similar results. It is worth mentioning that translating into Arabic using morphology-aware segmentation also requires de-segmentation and de-normalization of output which is no more required using a data driven segmentation approach and is merely an issue of combining segmented words together.



%The improvement in translation  system suffers from data sparseness and one advantage of segmentation is that it improves coverage of words. Another limitation of NMT comes because of the use of limited vocabulary which decreases the performance on the rare words translation. We suspect that segmentation can improve the rare words by splitting the morphologically rich words to smaller units.  
 
%In this paper, we analyze the 

%1) importance of segmentation and normalization
%2) importance in the context of machine translation - data sparsity, better word alignments, one of one mapping
%3) We explore NMT - how crucial is it to achieve similar quality without using any language dependent tools
%4) in results - training vs. quality, segmentation with respect to infrequent words
%5) analysis of output - how we were able to improve translation of specific words 
%6) experiment with different size of the data. May be for small data set, normalization is important
%7) Farasa applied on only infrequent words
%8) Farasa without normalization
%
% 9) No segmentation + No BPE + Normalization
% 10) No segmentation + BPE + Normalization
% 11) Farasa without Normalization
% 12) OOV analysis BPE vs. FARASA over testset
% Timing analysis
% MADA timing


%\section{Methodology}
%\label{sec:methodology}

\section{Segmentation Approaches}
\label{sec:segmentation}

\begin{comment}
We experiment with three segmentation schemes: i) morphology-aware segmentation, 
ii) %data driven-based 
%BPE-based 
sub-word segmentation
based on \texttt{BPE}, 
and iii) two variants of character-based segmentation. %character-level encoding and character CNN based encoding for Arabic word representations.
%Given 
For a source sentence $s={w_1, w_2, ... , w_N}$ and a target sentence $t={u_1, u_2, ... , u_M}$, we first map each source word to its corresponding segments depending on the segmentation scheme, %used, 
and then use the embedding of each segment for {\tt TRANSLATOR} which composed of standard encoder-decoder architecture with attention. 
\alert{\\YB: the preceding paragraph was confusing to me. It talks about segmentation schemes and then makes a sharp turn to translator, encoder-decoder, etc. I think we need some connecting material between these two topics. \\Alsot, I think the stuff about segmenter/embedder/translator (in minipage) is more confusing than helpful. It's enough to say that we embed the various segments in vector space and then feed them one-by-one to an encoder-decoder sequence-to-sequence model that is trained for translation or POS tagging. \\And then reference the beautiful figure.}
\resizebox{\linewidth}{!}{
\begin{minipage}{\linewidth}
  \begin{align*}
  &\text{Given } w_i \in s = \{w_1,w_2, ..., w_N\}, \text{we have} \\ %we've: } \\ % don't use abbreviations like we've
  &\texttt{SEGMENTER}(\tau) : \\
  & \texttt{\hphantom{bla}} \begin{cases}
      w_i \mapsto S_i =\{ w_i^1\} & \text{if } \tau \in A \\
      w_i \mapsto S_i =\{ w_i^1, ... , w_i^j\} & \text{if } \tau \in B \\
      \hphantom{.........} j=\text{len}(w_i) & \\
      w_i \mapsto S_i =\{ w_i^1, ... , w_i^j\} & \text{if } \tau \in  \Gamma \\
      \hphantom{.........} j=\text{num\_segments}(w_i) & \\
  \end{cases} \\
  & \text{where } A = \{\text{unsegmented}, \text{character-CNN}\} \\
  & \hphantom{where} B = \{\text{character}\} \\
  & \hphantom{where} \Gamma = \{\text{bpe, morphological}\} \\
  &\texttt{EMBEDDER}: S_i \mapsto E_i=\{v_i^1, v_i^2, ... v_i^j\} \\
  &\texttt{TRANSLATOR}: \{E_1, E_2, ..., E_N\} \mapsto t
  \end{align*}
\end{minipage}
}
\end{comment}

We experimented with 3 segmentation schemes: i) morphological segmentation, ii) sub-word segmentation based on \texttt{BPE}, 
and iii) two variants of character-based segmentation.
%Figure \ref{fig:segmentation} shows an example of a word under the above mentioned settings and its vector representations before the encoding layer. %In the following, we describe each method in detail.
%
 We first map each source word to its corresponding segments (depending on the segmentation scheme), %used, and then 
 embed all segments of a word in vector space and feed them one-by-one to an encoder-decoder sequence-to-sequence model. Figure \ref{fig:segmentation} illustrates the procedure. % for Arabic-to-English translation. For POS tagging, an additional embedding of POS tag of word under consideration is fed to the encoder-decoder model.

\begin{figure}[t] 
\centering
\includegraphics[width=0.95\linewidth]{segmentations-with-architecture.png}
\caption{An example of segmentation approaches for the word ``b\$rhm'' ``\<بشرهم>''; the blue vectors indicate the embedding vector(s) used before the encoding layer. The embeddings in the case of Character CNN is computed using a convolutional neural network \cite{KimAAAI1612489}.}
\label{fig:segmentation}
\end{figure}

\subsection{Morphological Segmentation}

%\alert{This is just reiterating what we said in the intro and citing all the segmenters. I think we should instead describe the pipeline of MADA-MIRA/Farasa. I added some lines at the end.}
%\alert{we may reduce following if needed}

There is vast amount of work on statistical segmentation for Arabic. %includes %rule-based analyzers \cite{beesley1989two,beesley1996arabic,buckwalter2002buckwalter,khoja2001apt}, light stemmers \cite{aljlayl2002arabic,darwish2007adapting}, and statistical segmenters 
%\cite{darwish2002building,habash2009mada+,diab2009second,darwish2014using,pasha2014madamira,monroe2014word,abdelali-EtAl:2016:N16-3}. 
Here we use the state-of-the-art Arabic segmenter MADAMIRA~\cite{PASHA14.593} and Farasa~\cite{abdelali-EtAl:2016:N16-3}. %for the segmentation of Arabic
%as our baselines.
MADAMIRA involves a morphological analyzer that generates a list of possible word-level analyses (independent of context). The analyses are provided with the original text to a {\tt Feature Modeling} component that applies %{\tt
an
SVM %} 
and %{\tt 
a language model %Language Model} 
to make predictions, which are scored by an {\tt Analysis Ranking} component. The scored analyses are then used to perform segmentation. %Although very accurate, MADAMIRA is slow to an extent that it cannot be used in a real-time translation. Even training a large scale system becomes cumbersome MADAMIRA takes several days to perform segmentation. See \newcite{abdelali-EtAl:2016:N16-3} for numbers. 
Farasa on the other hand is a light weight %ATB
segmenter, which ignores language model context and instead uses a variety of features and lexicons to segment the text. %data. %The downside of Farasa is that it cannot be used for English-to-Arabic MT as its corresponding de-tokenizer doesn't exist.

%The Arabic-to-English pipeline using morphology-aware segmenters involve normalization and segmentation of text in a pre-processing step. In the other translation direction, additionally a post-processing step is required to de-normalize and de-tokenize the output. Different segmenters come with slightly different normalization and segmentation schemes, thus a segmentor compatible post-processing step is required.

\subsection{Data Driven Sub-word Units}

%Several word classes such as transliterations, compounds and cognates can translated by decomposition into smaller units. Many researchers have capitalized on this intuition to overcome data sparsity and handling OOV words. Compound splitting \cite{Koehn:2003c} is an important pre-processing step when training German-English systems. Lemmatization has found to useful when translating morphologically rich languages \cite{fraser-EtAl:2012:EACL2012}. Character-based models have shown to help significantly in closely related language pairs \cite{nakov-tiedemann:2012:ACL2012short} and for translating unknown words \cite{durrani-EtAl:2014:EACL}. 
%Several word classes such as transliterations, compounds and cognates can be translated by decomposition into smaller units. %\newcite{google-nmt:2016} and 
%
A number of data-driven %-based 
approaches have been proposed in the literature to segment words into smaller units \cite{demberg:07,virpioja:13} and have been used %them 
%for 
to improve phrase-based MT \cite{Fishel10linguisticallymotivated,Stallard:2012:UMR}.
%almannai-EtAl:2014:ANLP2014
Recently, with the advent of neural machine translation, a few sub-word-based techniques have been proposed that segment words into sub-word units to tackle the limited vocabulary %issue 
and unknown word problems \cite{sennrich-haddow-birch:2016:P16-12,google-nmt:2016}. Segmentation 
%in terms of sub-word units 
comes as a byproduct of these methods. %They may not be linguistically correct.

In this work, we explore \emph{Byte-Pair Encoding} ({\tt BPE}), a data compression algorithm \cite{Gage:1994:NAD:177910.177914} as an alternative to morphological segmentation of Arabic.
%
%\newcite{sennrich-haddow-birch:2016:P16-12} used \emph{Byte Pair Encoding} (BPE), a data compression algorithm by \newcite{Gage:1994:NAD:177910.177914}, to capitalize on this intuition, and handled the %Neural MT has a known 
%unknown word problem in Neural Machine Translation.  
\texttt{BPE} splits words into symbols (a sequence of characters) and then iteratively replaces the most frequent symbols with their merged variants. In essence, frequent character n-gram sequences will be merged to form one symbol. The number of merge operations is controlled by a hyper-parameter {\tt OP} which directly 
%
%In this paper, we explore {\tt BPE} as an alternative to Arabic morphology-aware segmentation \alert{$\leftarrow$ FD: I think this sentence is unnecessary since we've mentioned this before}. 
affects the granularity of segmentation: %where 
a high value 
of {\tt OP} 
means coarse segmentation and a low value means fine-grained segmentation.
%We optimize {\tt OP} on a development set for the experiments. %used by the {\tt BPE} algorithm to optimize the granularity of segmentation. %For machine translation experiments, %we analyze the effect of sub-word segmentation in context of granularity and show that the neural machine translation system performs better when 
%We found that the optimal value 
%%of {\tt OP} 
%is achieved when the ratio of source to target tokens is equal or greater than 1, provided the boundary conditions i.e. no-segmentation and character-level segmentation are avoided (details in Section \ref{sec:experiments}). 

%They used the data driven based segmentation methods that split words into smaller known sub-word units. The benefits of the approach are two fold; fix rare word problem and do segmentation of words. In this paper, we investigate byte pair encoding ({\tt BPE}) compression \cite{Gage:1994:NAD:177910.177914} algorithm from the perspective of segmentation of Arabic. 

%which requires to be tuned. We explore BPE-based segmentation as an unsupervised alternative to conventional segmentation techniques as previously used. 



\subsection{Character-level Encoding}

Character-based embeddings have been explored %for the task of 
in neural machine translation \cite{charNMT2016:wang} to handle the unknown word problem. We explored them as an alternative to morphological segmentation. The advantage here is that character embeddings do not require any complicated pre- and post-processing step other than segmenting words into characters. The fully character-level encoder treats the source sentence as a sequence of letters, encoding each letter (including white-space) in the LSTM encoder. The decoding may follow identical settings. 
%encoding at character-level. \alert{YB: the last sentence isn't clear} 
In the work presented here, we restrict the character-level representation to the Arabic side of the parallel corpus and use words for the English side. Figure \ref{fig:segmentation} shows that %each character in a word is 
all source characters are 
encoded into %an 
embedding vectors which are then provided to the encoding layer. % in case of Arabic as source language. 

\paragraph{Character-CNN}
~\newcite{KimAAAI1612489} presented a neural language model that takes character-level input and learns word embeddings using a convolutional neural network over the characters. These embedding are then provided to the encoder as input. The intuition here is that the character-based word embedding should be able to learn the morphological phenomenon a word inherits. Compared to fully character-level encoding, here the encoder gets the word-level embeddings as in the case of unsegmented words (see Figure \ref{fig:segmentation}). However, the word embedding is intuitively richer than the embedding learned over unsegmented words because of the convolution over characters.
%We utilize a convolutional neural network over characters (\texttt{cCNN}), originally proposed by for sentence classification. This model is still aware of word boundaries, but instead of embedding words it embeds characters and runs multiple convolutional filters of different widths over the character vectors. 
In this work we use character-CNN to aid Arabic word segmentation. The method was previously shown to help German-English~\cite{costajussa-fonollosa:2016:P16-2} neural machine translation. %Arabic-Hebrew~\cite{belinkov:semat2016} and  \alert{\ND: Lets hold on to this citation for camera-ready}
 


\begin{table*}[!ht]
\centering
\footnotesize
\begin{tabular}{l|rrrr|r||rrrr|r}
\toprule
 & \multicolumn{5}{c||}{Arabic-to-English} & \multicolumn{5}{c}{English-to-Arabic} \\
\# SEG & tst11 & tst12 & tst13 & tst14 & AVG. & tst11 & tst12 & tst13 & tst14 & AVG. \\
\midrule
{\tt UNSEG} & 25.7 & 28.2 & 27.3 & 23.9 & 26.3 & 15.8 & 17.1 & 18.1 & 15.5 & 16.6 \\
\midrule
%MADA & 29.7 & 33.0 & 33.9 & 28.8 & 31.4 & 16.8 & 19.3 & 20.8 & 17.6 & 18.6 \\
%Farasa & 29.6 & 33.3 & 33.4 & 28.9 & 31.3 & - & - & - & - & -\\
%MORPH-norm & 29.6 & 33.3 & 33.4 & 28.9 & 31.3 & 16.8 & 19.3 & 20.8 & 17.6 & 18.6 \\
{\tt MORPH} & 29.2 & 33.0 & 32.9 & 28.3 & 30.9 & 16.5 & 18.8 & 20.4 & 17.2 & {\bf 18.2} \\
{\tt cCNN} & 29.0 & 32.0 & 32.5 & 28.0 & 30.3 & 14.3 & 12.8 & 13.6 & 12.6 & 13.3 \\
{\tt CHAR} & 28.8 & 31.8 & 32.5 & 27.8 & 30.2 & 15.3 & 17.1 & 18.0 & 15.3 & 16.4 \\
{\tt BPE}  & 29.7 & 32.5 & 33.6 & 28.4 & {\bf 31.1} & 17.5 & 18.0 & 20.0 & 16.6 & 18.0 \\ 
%Morfessor & 29.7 & 33.5 & 34.4 & 28.8 & 31.6 & 16.8 & 17.5 & 19.2 & 15.8 & 17.3 \\
%\midrule
%BPE-49.5k  & 29.3 & 32.3 & 33.0 & 28.0 & 30.7 & 17.4 & 17.6 & 18.9 & 15.9 & 17.5  \\
%BPE-49.5k$_{NORM}$  & 29.7 & 32.7 & 33.9 & 28.5 & 31.2 &  -&  -& - & - &- \\
\bottomrule
\end{tabular}
\caption{\label{tab:results-ar-en} Results of comparing several segmentation strategies. For BPE, we used an {\tt OP} value of 30 and 90 for Arabic to English and English to Arabic respectively}
%where {\tt MORP} is morphology-aware segmentation, {\tt cCNN} is using character CNN, {\tt Char} is using character-level representation. , and BPE-49.5 is sub-word segmentation with number of operations ({\tt OP}=49.5k)}
\end{table*}

\section{Experiments}
\label{sec:experiments}
%\subsection{Data Settings}
\paragraph{Data} The MT systems were trained on 1.2 Million sentences, a concatenation of TED corpus \cite{cettoloEtAl:EAMT2012}, 
LDC NEWS data, QED \cite{guzman-sajjad-etal:iwslt13} 
and an MML-filtered \cite{Axelrod_2011_emnlp} UN corpus.
%small 
%portion of a UN corpus \cite{ZiemskiJP16} selected through MML filtering \cite{Axelrod_2011_emnlp}. %We processed the English side of the corpus using the standard tokenizer of Moses ($\approx$ 28M tokens). 
%We tokenized the English side of the data using the standard Moses tokenizer. 
We used %concatenation of IWSLT 
dev+test2010 %and test-2010
for tuning and % used
%IWSLT 
tst11-14 %as test sets. 
for testing.
%
\paragraph{POS tagging} We used a concatenation of part 2 (v3.1) and part 3 (v3.2) of the Arabic Treebank
%, which contains 1100 distinct newswire stories from the Ummah Press 
%and the Lebanese publication An Nahar 
\cite{%maamouri2011atb2,
maamouri2011atb3}. %For training,
The data consists of 18268 sentences. 
%(483,909 words).
%(571,610 token). 
We %split it into 
used 80\% for training, 5\% for development and the remaining 
%15\% 
for test.

%\subsection{System Settings}

\paragraph{Segmentation} %For \textit{morphological segmentation} ({\tt MORPH}), 
We %initially used %both 
experimented with MADAMIRA and Farasa using ATB segmentation. %\footnote{We use the ATB segmentation scheme as it was shown to be superior to other schemes in Arabic-English MT~\cite{Kholy:Habash:2012,sajjad-etal:iwslt13}.} %However, since both of them perform very similar, we only report the
%However, in our initial experiments we found Farasa %was 
%performed slightly better, we only report experiments using Farasa, unless otherwise stated. \footnote{For English-to-Arabic, we used MADAMIRA since we do not have a detokenizer compatible with Farasa.}
%
%and BPE sub-word units. %~\cite{sennrich-haddow-birch:2016:P16-12}. 
In Arabic-to-English experiments, we found Farasa to perform slightly better and will therefore report that as a baseline. For English-to-Arabic, MADAMIRA performs significantly better. For {\tt BPE}, we tuned the value of merge operations {\tt OP} and found 30k and 90k to be optimal for Arabic-to-English and English-to-Arabic respectively.
%\alert{ND: this should be defined in the settings} For English-to-Arabic and Arabic-to-English directions, we found optimal value of {\tt OP} to be $90$ and $30$ respectively. Optimization was performed on test-2011.
%
In the case of \textit{no segmentation} ({\tt UNSEG}) and \textit{character-CNN} ({\tt cCNN}), we tokenized the Arabic text with the standard English tokenizer of Moses, which separates punctuation marks.
For \textit{character-level} encoding ({\tt CHAR}), we preserved word boundaries by replacing space with a special symbol and then separated every character with a space.

\paragraph{NMT Settings} We used {\tt seq2seq-attn}~\cite{kim2016}, a Torch-based implementation of NMT, where we employed a bidirectional LSTM encoder and an LSTM decoder, both with a size of 500. The implementation used the global-general-attention model with input-feeding~\cite{luong-pham-manning:2015:EMNLP}.
%\alert{cite}. 
We keep the sentence length limit to 100 for {\tt MORPH}, {\tt UNSEG}, {\tt BPE} and {\tt cCNN} experiments. For {\tt CHAR} experiments, we limit the sentence length to 500 characters. The source and target vocabulary is limited to 50k each. Both the encoder and the decoder have %are composed of 
2 LSTM layers.

\subsection{Machine Translation Results}

%We experimented with using morphological segmenter; MADA and Farasa ({\tt MORPH}), character CNN-based modeling ({\tt cCNN}) of Arabic words, character-level segmentation ({\tt CHAR}) of Arabic and data driven based sub-word unit segmentation ({\tt BPE}). Note that for all the experiments segmentation is applied on the Arabic side only. The English side is kept unprocessed apart from standard Moses tokenization. 
%For example, in case of BPE we segmented the Arabic side of the corpus using BPE and used English side constant for all experiments.
Table \ref{tab:results-ar-en} presents %the 
machine translation results using all %various 
segmentation strategies. Note that for all experiments, segmentation is applied on the Arabic side only. The English side is %kept unprocessed apart from standard Moses tokenization.
tokenized and true-cased using standard Moses pipeline and is constant across experiments.
%compares the results of Arabic-English machine translation systems while using various types of segmentation strategies for Arabic. 

Compared to the {\tt UNSEG} system,
%\alert{FD: No need for footnote anymore, I think its clear from previous section} \footnote{Arabic side is segmented for punctuation only.} 
the {\tt MORPH} system improved translation quality by 4.6 and 1.6 BLEU points in Arabic-to-English and English-to-Arabic systems respectively. The significant improvement in performance shows the importance of segmentation for Arabic MT. The results also improved by up to 3 BLEU points for {\tt cCNN} and {\tt CHAR} systems in the Arabic-to-English direction when compared with {\tt UNSEG} system. However, the performance is lower by at least 0.6 BLEU points compared to the {\tt MORPH} system. 

In the English-to-Arabic %other 
translation direction, where {\tt cCNN} and {\tt CHAR} are applied on the target side, the performance dropped significantly. In the case of {\tt CHAR}, %we speculate that 
mapping one source word to many target characters makes it harder for NMT to learn a good model. This is in line with our finding on using lower value of {\tt OP} for {\tt BPE} segmentation, %which is 
%described later in this section 
(See paragraph \textbf{Analyzing the effect of OP}). %A character-to-character system would be an option to prove our hypothesis. However, we did not try it because 1) it is out of the scope of the paper and 2) character-based systems are computationally expensive to train.
%and take 5x more time to train than a word-based NMT system. \alert{FD: I dont think we should mention this, this depends on a lot of factors - }
Surprisingly, the {\tt cCNN} system results were inferior to the {\tt UNSEG} system for English-to-Arabic. A possible explanation 
%for this phenomenon 
is that the decoder's predictions are still done at word level even when using the {\tt cCNN} model (which encodes the target input during training but not the output). In practice, this can lead to generating unknown words. Indeed, in the Arabic-to-English case {\tt cCNN} significantly reduces the unknown words in the test sets, while in the English-to-Arabic case the number of unknown words remains roughly the same between {\tt UNSEG}  and {\tt cCNN}. 

\alert{A sentence to conclude why BPE is performing good}
The {\tt BPE} system outperformed all other systems in the Arabic-to-English direction and is lower than {\tt MORPH} by only 0.2 BLEU points in the opposite %translation 
direction. We can therefore %To this end, we can 
conclude that machine translation involving the Arabic language achieves competitive results when the data-driven, {\tt BPE} segmentation is used. This 
comes with an additional benefit of \emph{language-independent} pre-processing and post-processing pipeline.


%We trained the {\tt BPE} systems using the optimum value of {\tt OP} obtained empirically, which is 30k and 90k for Arabic-to-English and English-to-Arabic respectively. %, that targets the infrequent words by splitting them into known sub-word units. We trained BPE on the unsegmented Arabic side of the training data. We restricted the number of operations ({\tt OP}) to 49500 considering the vocabulary size which is limited to 50k. 
%and applied it to Arabic side of the training and test data. 

%These results have major impact since they advocate a language independent pipeline of Arabic machine translation.

%better than the unsegmented system by 4.4 and 1.1 BLEU points for Arabic-to-English and English-to-Arabic translation directions respectively. It also out-performed the {\tt cCNN} and {\tt Char} systems in both translation directions. The results of using BPE are promising since it makes the Arabic translation pipeline completely language independent. However, this comes with a price of compromising on in achieving the best quality system (using morphology-aware segmentation). The BPE-based system is lower by 0.7 and 1.1 BLEU points compared to the best morphology-aware system\footnote{Because of the unavailability of the Farasa de-tokenizer and de-normalizer, we could not build an English-to-Arabic system based on Farasa.}.

%It is worth noting here that the morphology-aware segmenters normalize and segment the data. The other methods that we tried here such as character-based segmentation or BPE-based segmentation do not normalize the text. For the sake of completeness and to have equally comparable BPE-based system to the morphology-aware system, we normalized the training data and then used it for the BPE-based segmentation. The results (last row in Table \ref{tab:results-ar-en}) improved by 0.5 BLEU points and are only 0.1 and 0.2 BLEU points lower than the morphology-aware system. \alert{HS: EN2AR norm system}

%with unsegmented text and with using data driven based segmentation (BPE) to segment infrequent words. MADA and Farasa both segment and normalize the data. The NMT system achieved comparable performance of up to 31.4 BLEU points when used either of them for segmentation. The system trained on unsegmented Arabic (only tokenized for punctuation) dropped the results by 5.1 BLEU points. This is a significant drop in performance which shows the importance of word segmentation of Arabic. Later, we trained BPE on the unsegmented training data, separately for both source and target languages, restricting the number of operations ({\tt OP}) to 49500 (as recommended by \cite{sennrich-haddow-birch:2016:P16-12}) and applied it to Arabic side of the training and test data only ($BPE-S$) and to both Arabic and English side of the training and test data ($BPE$). 

\paragraph{Analyzing the effect of OP:}
The unsegmented training data consists of 23M Arabic tokens and 28M English tokens. The parameter {\tt OP} decides the granularity of segmentation: %where 
a higher value of {\tt OP} means fewer segments. For example, at {\tt OP}=50k, the number of Arabic tokens is greater by 7\% compared to {\tt OP}=90k. We tested four different values of {\tt OP} (15k, 30k, 50k, and 90k) and analyzed its effect with respect to the number of tokens in English (28M tokens) and the quality of translations produced.
Figure \ref{fig:ar-en} summarizes our findings on test-2011 dataset, where x-axis presents the ratio of source to target language tokens and y-axis shows the BLEU score. The boundary values for segmentation are character-level segmentation and unsegmented text which can be seen as BPE with {\tt OP}=0 and {\tt OP}=$N$ respectively, where $N$ is the number of types in the unsegmented corpus.
%\alert{FD: do you think instead of saying bpe=120k, a better representation is bpe=vocab\_size or bpe=$\infty$ (since this 120k number seems to be out of no where to the reader)} respectively. 
For both language directions, we observed that a source to target token ratio close to 1 and greater works best provided that the boundary conditions (unsegmented Arabic and character-level segmentation) are avoided. In the English-to-Arabic %translation 
direction, the system improves for coarse segmentation whereas in the Arabic-to-English %translation 
direction, a much finer-grained segmentation of Arabic performed better. These findings are in line with the ratio of tokens generated using the {\tt MORPH} systems (28.7M Arabic tokens). Generalizing from the perspective of neural machine translation, the system learns better when total numbers of source and target tokens are close to each other. The system shows better tolerance towards modeling many source words to a few target words compared to the other way around.
%\alert{YB: it's remarkable that AR/EN 4.37 ratio still keeps good BLEU close to the best, while En/AR 1.25 already drops BLEU a lot. Any thoughts why?}

%We can hypothesize that in translating English to Arabic segmentation only helps to reduce the problem of data sparseness. The information which is missing from the morphologically poor language source language can not be recovered. 

%We analyzed the number of tokens produced using BPE vs.  and their effect on the quality of machine translation. 
%
%compared them with the tokens produced by morphology-aware segmenters. 
%
%Out of 23M tokens on the Arabic side of the training data, only 14\% tokens got segmented by BPE with {\tt OP}=50k. This is 7\% less than the number of tokens produced by morphology-aware segmenters. 
%
%We tested four different values of {\tt OP}=15k, 30k, 50k, 90k. % and observed it's effect on the quality of machine translation. 
%Table \ref{tab:results-ar-en-bpe} shows the statistics and the results. 
%number of tokens produced by different values of {\tt OP}. 
%%Analyzing further from the perspective of morphology-aware segmentation, at {\tt OP}=30k the number of tokens produced by {\tt BPE} are close to the ones produced by {\tt MORPH}. The Arabic to English system performed best at {\tt OP}=30k. In case of English to Arabic system, the system at {\tt OP}=30k is a lot better than unsegmented Arabic and is lower by only 0.4 BLEU points from the best BPE-based system. \alert{FD: This paragraph seems a bit blurry - I think we should add more discussion, or atleast a conclusion from this finding}


%The Arabic-to-English system achieved the best performance and is only 0.3 BLEU points behind Farasa. It is worth mentioning here that the morphology-aware segmentation systems have an additional advantage of normalizing Arabic text. For Arabic-to-English direction, we also observed a variation in BLEU score with varying {\tt OP}. However, trend is different. The system performance improved with fewer number of operations and the best performance is achieved at {\tt OP}=90k.

%To further understand the relationship between segmentation granularity and the quality of the system, we analyzed the ratio of source versus target tokens in relation to the quality of the system. Figure \ref{fig:ar-en} plots the ratio of number of tokens (x-axis) and BLEU score (y-axis) of fully segmented system (character-level) to unsegmented system. The performance of the NMT system improves with a source to target ratio of one and greater provided the boundary conditions of no-segmentation and character-level segmentation is avoided. 

%performs best when there exist at least one to one and preferably one to many mappings between source and target tokens provided avoiding the boundary cases of fully segmented text at character-level and unsegmented text.


%This is also close to the total number of tokens in the English side of the training corpus (28.1 million). 
%Figure \ref{fig:ar-en} shows the effect of using several granular level of segmentation, starting from characters to completely unsegmented text, on the BLEU score. The x-axis presents the number of Arabic tokens produced (in millions) and y-axis shows the BLEU scores. There is a consistent overall trend for both language directions i.e. sub-word level segmentation is required to achieve high quality translations. However, peak is different for both directions. The Arabic-to-English system achieved best results when segmentation is achieved using BPE with {\tt OP}=30k whereas in the other direction, {\tt OP}=90k performed best. Looking at numbers from the perspective of source versus target number of tokens, it is observed that the NMT system performs better when source to target token ratio is 

\begin{figure} 
\centering
\includegraphics[width=\linewidth]{ar-en-bar.png}
\caption{Source to target token ratio with varying {\tt OP} versus BLEU score. Character and unsegmented systems can be considered as {\tt BPE} with {\tt OP}=0 and {\tt OP}=$N$ respectively}
\label{fig:ar-en}
\end{figure}

%\begin{figure} 
%\centering
%\includegraphics[scale=0.35]{en-ar-graph.png}
%\caption{EN-AR}
%\label{fig:en-ar}
%\end{figure}


%\alert{YB: the last part, about the fraction of segmented words, is nice. Perhaps it will be good to bar-plot the fraction of segmented words for each method next to the BLEU improvement\\HS: will do that}

%BPE resolves the issue of unknown words by splitting them into known sub-word units. In the case of morphology-aware system, there are still 1.5\% unknown words in the test set. In order to handle unknown words from system 1 and 2, we trained BPE (no. of operations 49.5k) on the segmented data and applied it. The results improved by 1 BLEU points compared to their respective baseline.

%To summarize, the MT system trained only on the BPE-segmented data achieved comparable results (only 0.2 BLEU points lower) to the best morphology-aware system. Normalization of the data further improved the BPE-segmented system but with an addition of language dependent processing. In order to get the best out of morphology-aware segmentation and BPE, both should be applied.

\begin{comment}


\begin{table}
\centering
\footnotesize
\begin{tabular}{l|rrrr|c}
\toprule
 & \multicolumn{4}{c}{BPE {\tt OP}} & MORPH \\
 & 90k & 50k & 30k & 15k & - \\%& 49.5 \\
\midrule
TK. AR(M) & 25.0 & 26.2 & 27.7 & 32.4 & 27.8 \\ %& 28.7 \\
%TK. EN(M) & 28.3 & 28.6 & 29.2 & 31.8 & 28.1 & 28.6 \\
\midrule
%TY. AR(K) & 90.0 & 49.3 & 30.4 & 15.6 & 251 & 49.5 \\
%TY. EN(K) & 85.6 & 48.8 & 30.1 & 15.5 & 181 & 48.8 \\
%\midrule
AR-EN & 28.6 & 30.7 & 31.1 & 31.0 & 30.9 \\ %& 32.4 \\
EN-AR & 18.0 & 17.5 & 17.6 & 17.0 & 18.2 \\ %& 32.4 \\
\bottomrule
\end{tabular}
\caption{\label{tab:results-ar-en-bpe} Comparing the number of tokens produced by different values of {\tt OP} and Farasa}
\end{table}
%bpe40000 - ar 26.8 en 28.8
%full tokens - ar 23.2 en 28.1
\end{comment}

\begin{comment}

\begin{table} 
\centering
\footnotesize
\begin{tabular}{l|rrrr|r}
\toprule
\# SEG & tst11 & tst12 & tst13 & tst14 & AVG. \\
\midrule
1. MADA & 29.7 & 33.0 & 33.9 & 28.8 & 31.4 \\
2. Farasa & 29.6 & 33.3 & 33.4 & 28.9 & 31.3 \\
\midrule
BPE 15k-S  & 29.4 & 32.5 & 33.5 & 28.6 & 31.0 \\
BPE 30k-S  &  &  &  &  & 31.1  \\
BPE 49k-S  & 29.3 & 32.3 & 33.0 & 28.0 & 30.7  \\
BPE 90k-S  & 29.0 & 32.4 & 33.2 & 27.8 & 30.6  \\
\midrule
3. cCNN-S & 29.0 & 32.0 & 32.5 & 28.0 & 30.3 \\
3. cCNN-ST &  &  &  &  &  \\
3. Char-S &  &  &  &  &  \\
3. Char-ST &  &  &  &  &  \\
\midrule
3. Unsegmented & 25.7 & 28.2 & 27.3 & 23.9 & 26.3 \\
3. BPE-S &  &  &  &  &  \\
4. BPE & 29.6 & 32.7 & 33.6 & 29.0 & 31.2 \\
5. Norm-BPE & 30.5 & 33.0 & 34.4 & 30.2 & 32.0 \\
\midrule
6. MADA+BPE & 30.7 & 33.5 & 34.9 & 30.2 & 32.3 \\
7. Farasa+BPE & 30.8 & 33.3 & 35.0 & 30.5 & 32.4 \\
\midrule
BPE 15k both  & 30.2 & 32.5 & 33.3 & 28.8 & 31.2 \\
BPE 30k both  & 28.8 & 31.8 & 32.5 & 27.4 & 30.1  \\
BPE 49k both  & 29.6 & 32.7 & 33.6 & 29.0 & 31.2 \\
BPE 90k both  & 29.7 & 32.4 & 33.8 & 28.7 & 31.2 \\
\midrule
\midrule
BPE 30k-49k  & 30.5 & 32.8 & 33.8 & 29.5 & 31.7  \\
BPE 30k-90k  & 30.6 & 33.1 & 33.9 & 29.8 & 31.9 \\
\bottomrule
\end{tabular}
\caption{\label{tab:results-ar-en} Results of comparing morphology-aware segmentation with BPE-based segmentation ({\tt OP}=49.5k) for Arabic to English translation where $S$ presents only source side segmentation like BPE-S means BPE applied to Arabic only}
\end{table}



%\begin{table}
%\centering
%\footnotesize
%\begin{tabular}{l|rrrr|r}
%\toprule
%BPE & tst11 & tst12 & tst13 & tst14 & AVG.\\
%\midrule
%49500 & 29.6 & 32.7 & 33.6 & 29.0 & 31.2 \\
%30000 & 28.8 & 31.8 & 32.5 & 27.4 & 30.1 \\
%15000 &  &  & & & \\
%\bottomrule
%\end{tabular}
%\caption{\label{tab:results-ar-en-bpe} }
%\end{table}

\end{comment}

%\paragraph{Effect of varying {\tt OP}:}
%\alert{YB: this paragraph was not so clear to me}
%We observed the number of tokens produced by BPE vs. using a morphology-aware segmentor and analyzed them in the context of the number of tokens on the English side. The unsegmented Arabic and English corpus consisted of 23M and 28.1M tokens respectively. The morphology-aware segmentation increased the number of tokens to 27.8M which is relatively close to the number of tokens in English. On the other hand, the BPE-segmented data with {\tt OP}=49.5k has far less number of tokens. We hypothesized that finding a good ratio between the total number of Arabic and English tokens might help to learn better alignments and may further improve the quality of machine translation. 

%To test out hypothesis, we varied {\tt OP}=15k, 30k, 49.5k and 90k and analyzed the resulting number of tokens. 

%Out of 23M tokens in the Arabic side of the training data, BPE with {\tt OP}=49.5k segmented 7.5\% of the tokens. This is 15\% less than the morphology-aware segmentation.
 
%To further investigate our claim that splitting of infrequent words for machine translation is more important than the segmentation of all possible words of Arabic, we test with different values of {\tt OP} in BPE. 
%%The Arabic training data consists of 0.6M vocabulary types. 
%We chose {\tt OP}$= 90k$, $49.5k$, $30k$ and $15k$. A lower value of {\tt OP} reflects fine grained segmentation. Table \ref{tab:results-ar-en-bpe} shows the stats on the number of tokens and types achieved for each variation of {\tt OP} and presents the average BLEU scores. It is interesting to see that with fine-grained sub-word level segmentation, the performance of the MT system dropped. The other argument in favor of segmentation that it improves source word to target word mapping between Arabic and English does not look very convincing either. The number of source and target tokens are the closest in case of {\tt OP}$=15k$ and Farasa but results differ since a ratio close to 1 is hurting in the former case. This could be because of the over-segmentation of words as can be seen by comparing the total number of tokens in each set. **discussion on 90k is missing** In order to find a good balance between the total number of tokens generated for both English and Arabic and ratio between English and Arabic tokens, we used {\tt OP}$=90$ for English and {\tt OP}$=30$ for Arabic. 

%\paragraph{Effect of training set size:}
%Th*** Since we are using a reasonably large size of the data for training, it can be the case that morphology-aware segmentation is more helpful when training data is small and most of the words are infrequent in the data. We test this hypothesis by taking random samples of 30\% and 60\% of the training data and repeat the experiments presented in Table \ref{tab:results-ar-en}. 

%*** We analyzed the words segmented by the BPE. ***

%\paragraph{Training time comparison:}

\begin{comment}

\end{}
\begin{table} 
\centering
\footnotesize
\begin{tabular}{l|rrrr|r}
\toprule
\# SEG & tst11 & tst12 & tst13 & tst14 & AVG. \\
\midrule
1. MADA & 16.4 & 18.3 & 19.7 & 16.5 & 17.7 \\
\midrule
3. cCNN-T &  &  &  &  &  \\
%3. cCNN-ST &  &  &  &  &  \\
3. Char-T & 15.3 & 17.1 & 18.0 & 15.3 & 16.4 \\
%3. Char-ST &  &  &  &  &  \\
\midrule
3. Unsegmented & 13.7 & 14.1 & 14.7 & 12.4 & 13.7 \\
4. BPE AR 30k & 17.1 & 17.7 & 19.5 & 16.1 & 17.6 \\
4. BPE AR 49k & 17.4 & 17.6 & 18.9 & 15.9 & 17.5 \\
%5. Norm-BPE &  &  &  &  &  \\
\midrule
6. MADA+BPE & 16.9 & 19.1 & 21.0 & 17.4 & 18.6 \\
4. BPE both 49k& 17.5 & 18.0 & 20.0 & 16.6 & 18.0 \\
\bottomrule
\end{tabular}
\caption{\label{tab:results-en-ar} Results of comparing morphology-aware segmentation with BPE-based segmentation for English to Arabic translation }
\end{table}
\end{comment}


==> methodology.tex <==

We experiment with three segmentation schemes: i) morphological segmentation, ii) sub-word segmentation based on \texttt{BPE}, 
and iii) two variants of character-based segmentation. Consider Arabic-to-English translation direction, given a Arabic sentence we segment it using 


For a source sentence $s={w_1, w_2, ... , w_N}$ and a target sentence $t={u_1, u_2, ... , u_M}$, we first map each source word to its corresponding segments depending on the segmentation scheme, %used, 
and then embed all segments of a word in vector space and feed them one-by-one to an encoder-decoder sequence-to-sequence model. Figure \ref{fig:segmentation} illustrates the procedure. For POS tagging, an additional embedding of POS tag is fed to the encoder-decoder model.



use the embedding of each segment for {\tt TRANSLATOR} which composed of standard encoder-decoder architecture with attention. 
we embed the various segments in vector space and then feed them one-by-one to an encoder-decoder sequence-to-sequence model that is trained for translation or POS tagging.
\resizebox{\linewidth}{!}{
\begin{minipage}{\linewidth}
  \begin{align*}
  &\text{Given } w_i \in s = \{w_1,w_2, ..., w_N\}, \text{we have} \\ %we've: } \\ % don't use abbreviations like we've
  &\texttt{SEGMENTER}(\tau) : \\
  & \texttt{\hphantom{bla}} \begin{cases}
      w_i \mapsto S_i =\{ w_i^1\} & \text{if } \tau \in A \\
      w_i \mapsto S_i =\{ w_i^1, ... , w_i^j\} & \text{if } \tau \in B \\
      \hphantom{.........} j=\text{len}(w_i) & \\
      w_i \mapsto S_i =\{ w_i^1, ... , w_i^j\} & \text{if } \tau \in  \Gamma \\
      \hphantom{.........} j=\text{num\_segments}(w_i) & \\
  \end{cases} \\
  & \text{where } A = \{\text{unsegmented}, \text{character-CNN}\} \\
  & \hphantom{where} B = \{\text{character}\} \\
  & \hphantom{where} \Gamma = \{\text{bpe, morphological}\} \\
  &\texttt{EMBEDDER}: S_i \mapsto E_i=\{v_i^1, v_i^2, ... v_i^j\} \\
  &\texttt{TRANSLATOR}: \{E_1, E_2, ..., E_N\} \mapsto t
  \end{align*}
\end{minipage}
}

==> seg-analysis.tex <==

\section{Discussion}
\label{sec:analysis}
We analyzed the segmentation produced by {\tt BPE} at {\tt OP}=30k and {\tt MORPH}. It is observed that BPE segments words into larger sub-word units compared to Farasa which segments based on the morphology of Arabic. %We observed that the segmentation using BPE is close to what can be achieved using unsupervised stemming while trying to find the most common affix. 
Some of the segmentation makes a valid decomposition but others create more ambiguity. 
As shown in Table \ref{tab:bpesegs}, segmentations such as  \<رة> \<الخط> ``AlxT rp'', and  \<بها> \<قترا> \<وا> ``wA qtrA bhA'' produces some valid segments. There other segments that will deviate and alter the word by generating words that are not related to the original word; as the case for the resulting affixes in the above examples \<الخط> ``AlxT''(the line), \<بها> ``bhA'' (with it). The decomposition might help maximizing the vocabulary compression but might also generated unwanted segments which have different semantics than the original word and impact negatively the overall distribution of the tokens.    
%considering we do not drop any stems here. 
%Since it has no linguistic information. For example, the word *** 's linguistically correct segmentation is *** but BPE over-segment it as ..
\begin{comment}
\begin{table*}
\centering
\small
\begin{tabular}{cccc}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
{\bf Word} & {\bf Buckwalter} & {\bf Gloss} & {\bf MORPH} & {\bf MORF} & {\bf BPE-30k} & {\bf BPE-15k} & {\bf BPE-5k}\\\hline
\<الخطرة> & AlxTrp & the dangerous & \<ال خطر ة> & \<ال خطر ة> & \<الخطرة> & \<الخطرة> &  \<رة> \<الخط> \\
\<ويهدف> &  wyhdf &  and aims to & \<و يهدف> & \<و ي هدف> & \<ويهدف> & \<هدف> \<وي>  & \<هدف> \<وي> \\
\<وتمكين> & wtmkyn & and to enable & \<و تمكين> & \<و تمكين> &\<وتمكين> & \<وتمك> \<ين> &  \<ين > \<مك> \<وت>   \\
\<واقترابها> & wAqtrAbhA & and its closeness & \<و اقتراب ها> & \<و اقتراب ها> & \<بها> \<قترا> \<وا> & \<بها> \<قترا> \<وا>   & \<بها> \<قترا> \<وا>\\
\<المديونيات>  & AlmdywnyAt & the debts  & \<ال مديوني ات> & \<ال مديونيات> & \<المديونيات> & \<ونيات>  \<المدي> &  \<يات> \<ون> \<دي>  \<الم> 
\\\hline
\end{tabular} 
\end{tabular} 
\caption{BPE Segmentation versus MORPH}\label{tab:bpesegs}
\end{table*}

\end{comment}

%For end-to-end machine translation, one advantage of BPE is to segment unknown words into known words. However, this brings an issue of segmenting proper names that should be transliterated rather than translated from known sub-word units. We found that 

%Here we compare the segmentation generated by Farasa and BPE. This can go into previous section too.
%Figure~\ref{fig:seg-example} illustrates the differences between supervised morphology-aware segmentation (Farasa) and unsupervised data-driven segmentation (BPE). Segmenting with morphological knowledge leads to meaningful sub-word units, as indicated by the glosses. In contrast, BPE does not respect morpheme boundaries and its sub-word units do not always coincide with meaningful morphemes. 

%\begin{figure*}[t]
%\begin{tabular}{l l}
%Unsegmented & wsnqwm bAxbArkm bbED AlqSS mn AlbHr hnA fy Alfydyw \\
%BPE & wsnqwm bAx+ bArkm bbED AlqSS mn AlbHr h+ nA fy Alfydyw \\
%Farasa & ws+ nqwm b+ AxbAr +km b+ bED AlqSS mn AlbHr hnA fy Alfydyw \\
%Gloss & and-will we-do PREP-tell you PREP some the-stories from the-sea here in the-video\\
%Translation & "And we're going to tell you some stories from the sea here in video" \\
%\end{tabular}
%\label{fig:seg-example}
%\caption{Example segmentations of supervised morpohlogy-aware Farasa and unsupervised data-driven BPE.}
%\end{figure*}
